Detecting Outliers with Poisson Image Interpolation

Supervised learning of every possible pathology is unrealistic for many primary care applications like health screening. Image anomaly detection methods that learn normal appearance from only healthy data have shown promising results recently. We propose an alternative to image reconstruction-based and image embedding-based methods and propose a new self-supervised method to tackle pathological anomaly detection. Our approach originates in the foreign patch interpolation (FPI) strategy that has shown superior performance on brain MRI and abdominal CT data. We propose to use a better patch interpolation strategy, Poisson image interpolation (PII), which makes our method suitable for applications in challenging data regimes. PII outperforms state-of-the-art methods by a good margin when tested on surrogate tasks like identifying common lung anomalies in chest X-rays or hypo-plastic left heart syndrome in prenatal, fetal cardiac ultrasound images. Code available at https://github.com/jemtan/PII.

==> oldTables.tex <==
\iffalse
\begin{table}[ht]

\centering 
%\setlength{\tabcolsep}{5pt}
\begin{tabular}{c c c c c }
%\hline\hline   
\toprule
\multicolumn{2}{c}{\multirow{1}{*}{\textbf{Dataset}}} &
\thead{\textbf{Normal}\\ \textbf{Train}} & 
\thead{\textbf{Normal}\\ \textbf{Test}} & 
\thead{\textbf{Anomalous}\\ \textbf{Test}} \\ %[0.5ex]

\midrule
\multicolumn{1}{c}{\multirow{2}{*}{Chest X-ray}} & Male PA & 17852 & 2634 & 3366 \\
\multicolumn{1}{c}{\multirow{1}{*}{}} & Female PA & 14720 & 2002 & 2748 \\ 
 
\multicolumn{1}{c}{\multirow{2}{*}{Fetal US}} & 4CH & $283\times20$ & $34\times20$ & $54\times20$\\
\multicolumn{1}{c}{\multirow{1}{*}{}} & 3VT & $225\times20$ & $35\times20$ & $38\times20$ \\

%[1ex]      
\bottomrule
\end{tabular}
\caption{Number of images in each data partition.}
\label{table:NumImages}
\end{table}
\fi



\iffalse
\begin{table}[ht]

\centering 
\setlength{\tabcolsep}{5pt}
\begin{tabular}{c c|c c c c |c}
\toprule
%\hline\hline                        
\multicolumn{2}{c|}{\multirow{1}{*}{\textbf{Dataset}}} &
\thead{\textbf{Deep}\\ \textbf{SVDD}} & 
\thead{\textbf{VQ-}\\ \textbf{VAE2}} & 
\textbf{FPI} & \textbf{PII} & \textbf{Supervised} \\ %[0.5ex]

\midrule
\multicolumn{1}{c}{\multirow{2}{*}{Chest X-ray}} & Male PA &
0.565 & 0.503 & 0.533 & 0.690 & \\
\multicolumn{1}{c}{\multirow{1}{*}{}} & Female PA & 
0.556 & 0.516 & 0.586 & 0.703 & \\
 
\multicolumn{1}{c}{\multirow{2}{*}{Fetal US}} & 4CH & 
0.685 & 0.617 & 0.658 & 0.723 & \\
\multicolumn{1}{c}{\multirow{1}{*}{}} & 3VT & 
0.893 & 0.578 & 0.710 & 0.929 & \\

%[1ex]      
\bottomrule
\end{tabular}
\caption{Average Precision for each dataset and method.}
\label{table:AvgPrecision}
\end{table}
\fi





\begin{table}[ht]
\centering 
\begin{tabular}{l c c c c c}
\toprule
\multirow{2}{*}{\textbf{Dataset}}
& \multicolumn{3}{c}{{Chest X-ray}} &  \multicolumn{2}{c}{{Fetal US}} \\
 \cmidrule(lr){2-4}
 \cmidrule(lr){5-6}
& \textbf{\mars PA} & \textbf{\female PA} & & \textbf{4CH} & \textbf{3VT} \\
%\cmidrule(lr){2-5}
\midrule
 & \multicolumn{5}{c}{number of images} \\
 %\cmidrule(lr){2-6}
\cmidrule(lr){2-4} 
\cmidrule(lr){5-6}
Normal Train & 17852 & 14720 & & 283 $\times$ 20 & 225 $\times$ 20 \\
Normal Test & 2634 & 2002 & & 34 $\times$ 20 & 35 $\times$ 20 \\
Abnormal Test & 3366 & 2748 & & 54 $\times$ 20 & 38 $\times$ 20 \\
\midrule
 & \multicolumn{2}{c}{Avg Precision} & \multicolumn{1}{c}{IoU} & \multicolumn{2}{c}{Avg Precision} \\
 \cmidrule(lr){2-4} 
 %\cmidrule(lr){4-4}  
 \cmidrule(lr){5-6}
Deep SVDD & 0.565 & 0.556 & XX & 0.685 & 0.893 \\
VQ-VAE2 & 0.503 & 0.516 & XX & 0.617 & 0.578 \\
FPI & 0.533 & 0.586 & XX & 0.658 & 0.710 \\
PII & \textbf{0.690} & \textbf{0.703} & XX & \textbf{0.723} & \textbf{0.929} \\
%\midrule
%Supervised & XX & XX & - & XX & XX \\
\bottomrule
\end{tabular}
\caption{Each dataset is presented in one column. The train-test split is shown for each partition (top). Note that ultrasound images are extracted from videos as 20 frame clips. Average precision is also listed for each method (bottom).}
\label{table:results}
\end{table}

